Katakomba: Tools and Benchmarks for Data-Driven NetHack

NetHack is known as the frontier of reinforcement learning research where learning-based methods still need to catch up to rule-based solutions. One of the promising directions for a breakthrough is using pre-collected datasets similar to recent developments in robotics, recommender systems, and more under the umbrella of offline reinforcement learning (ORL). Recently, a large-scale NetHack dataset was released; while it was a necessary step forward, it has yet to gain wide adoption in the ORL community. In this work, we argue that there are three major obstacles for adoption: resource-wise, implementation-wise, and benchmark-wise. To address them, we develop an open-source library that provides workflow fundamentals familiar to the ORL community: pre-defined D4RL-style tasks, uncluttered baseline implementations, and reliable evaluation tools with accompanying configs and logs synced to the cloud.

==> code/buffer.tex <==
\vspace{-0.1in}
\begin{python}[caption={Usage example: Katakomba provides a sequential replay buffer that one can use as an example of writing their own custom implementations.}]
buffer = SequentialBuffer(
    dataset=dataset,
    seq_len=your_seq_len,
    batch_size=your_batch_size,
    seed=your_train_seed,
    add_next_step=True       # useful for ORL algorithms, can be turned off for BC
)
\end{python}
